Increasing Validity Through Replication: An Illustrative TDD Case

Context: Software Engineering (SE) experiments suffer from threats to validity that may impact their results. Replication allows researchers building on top of previous experiments' weaknesses and increasing the reliability of the findings. Objective: Illustrating the benefits of replication to increase the reliability of the findings and uncover moderator variables. Method: We replicate an experiment on Test-Driven-Development (TDD) and address some of its threats to validity and those of a previous replication. We compare the replications' results and hypothesize on plausible moderators impacting results. Results: Differences across TDD replications' results might be due to the operationalization of the response variables, the allocation of subjects to treatments, the allowance to work outside the laboratory, the provision of stubs, or the task. Conclusion: Replications allow examining the robustness of the findings, hypothesizing on plausible moderators influencing results, and strengthening the evidence obtained.

==> text.tex <==
However, some limitations of the approach of Munir et al. should be considered when interpreting the results: (1) giving the same weight to every study within the same category may bias the results: different types of empirical studies and sample sizes may provide findings with different degrees of maturity; (2) inconclusive results might stem from poor designs (low rigour) but could, in the case of experiments, also be due to a low statistical power; (3) reporting style has a significant impact on the category into which the study falls, as a study with high quality reporting could be poorly designed; (4) the boundaries for relevance and rigour scores are fuzzy.

The systematic variation of context variables to neutralize previous experiments' threats may aid to overcome the limitations of the findings. 

Studies on TDD have yielded diverse results with regards to quality \cite{rafique2013effects}\cite{munir2014considering}\cite{shull2010we}: from improvements \cite{ficco2011bug}\cite{george2004structured}, to inconclusive results \cite{janzen2008does}\cite{pancur2003towards}, and to decreases in quality compared to traditional coding approaches \cite{muller2002experiment}. 

Along this article we use our illustrative example to argue that the threats to validity of the experiments on TDD may have potentially increased the heterogeneity of results observed so far. Identifying, isolating and uncovering the potential influence of such validity threats may aid to stabilize the results observed across the experimental path. Also to ease the acquisition of reliable knowledge. 

With our replication we aim to expand the validity of the evidence obtained.

We run a replication of Erdogmus et al.'s experiment on TDD \cite{erdogmus2005effectiveness}. Erdogmus et al.'s experiment was already closely replicated by Fucci et al. \cite{fucci2013replicated}. Erdogmus et al.'s and Fucci et al.'s experiments show a non-significant difference between the performance of TDD and iterative test last (i.e., ITL, the reverse approach of TDD, a development process that enforces the creation of software systems by means of small coding-testing-refactoring cycles). 

Since we think no metric is free from criticism, the exercise of different metrics for the same response variable may aid to increase the construct validity of new replications and eventually increase the reliability of the joint findings

As we can see in Table \ref{tab:settings_baseline_replications}, several elements were modified along the experimental path. By changing such elements, researchers are able to avoid the potential heterogeneity of results resulting from the materialization of previous threats to validity. Observing consistency of findings across replications may suggest that previous threats to validity did not materialized. Contrariwise, observing deviations across replications may point towards the plausible materialization of previous threats to validity. In the following section, we discuss threats to validity in BE and RE1 that can be overcome by a new replication and, on the way, learn context or moderator variables that may have an impact on the findings.

The within-subjects design also increases the similarities between groups since differences among individuals are fully cancelled out: subjects are all matched with themselves, cancelling out any inherent variability and greatly increasing power \cite{shadish2002experimental}. Our participants used the two treatments twice, thus avoiding the threat of achieving outlying results by chance; due to the "regression to the mean" effect, subjects achieved an average outcome closer to reality. 


Here we describe RE2's experimental design. 

\subsection{Research Questions}
\label{research_objectives}

The following research question drives RE2 (RE2.RQx):
\begin{itemize}
    \item{\textbf{RE2.RQ}: Do programmers produce TDD and ITL perform similarly in terms of \textbf{quality}?}
\end{itemize}

As we overcame the mono-operation bias threat of BE and RE1 by including multiple tasks, we needed to include another research question in our replication:
\begin{itemize}
    \item{\textbf{RE2.RQ2}: Do TDD and ITL perform similarly in terms of \textbf{quality} across \textbf{tasks}?}
\end{itemize}	

\subsection{Variables and Hypotheses}
\label{variables}

The main independent variable of our experiment is \textbf{development approach} with \textit{TDD} and \textit{ITL} as treatments. Subjects follow these development approaches to complete four different tasks (one different task per experimental session), two tasks with each treatment.

Another independent variable of the experiment is \textbf{experimental task}: we want to analyse whether the task moderates the effects produced by TDD on the dependent variable. This factor has four levels in our experiment: \textit{MR, BSK, MF,} and \textit{SDK} (described thoroughly in Section \ref{experimental_objects_tasks}).

The dependent variable in the current study is \textbf{quality}. This variable is measured by means of acceptance test suites developed by the experimenters for MR, MF and SDK and inherited from RE1 for BSK.

As discussed in Section \ref{response_variables}, quality is represented in our experiment by functional correctness (i.e., a quality sub-characteristic defined in ISO 25010 \cite{iso25010}). We measure QLTY as the total of number of asserts that pass divided by the total number of task's asserts. QLTY shows how much quality work overall has been performed by a developer. Therefore, it takes into account not only the quality of the work delivered ($\#Assert(pass)$) but as well the total amount of work to be done ($\#Assert(all)$). 



Table \ref{null_hypotheses_experiment} shows the null hypotheses of this experiment.

\begin{table}[h!]
\small
\caption{Null hypotheses of the current replication.}
\label{null_hypotheses_experiment}
\begin{center}
\begin{tabular}{c|c|p{5cm}|l} \hline
    \textbf{RE2.RQ} & \multicolumn{2}{c}{\textbf{Null hypothesis}} & \textbf{Response Variable}\\ \hline \hline
    \multirow{1}{*}{RE2.RQ1}  &$\mathbf{H_{101}}$&There is no difference in QLTY when applying TDD or ITL. & Dev. Approach  \\ \hline
    RE2.RQ2  &$\mathbf{H_{201}}$&There is no difference in QLTY when applying TDD or ITL regardless of the task & Dev. Approach * Task \\\hline
\end{tabular}
\end{center}
\end{table}

\subsection{Design}
\label{design}
The experiment was embedded in a five-day training course. The training sessions included several ITL and TDD practice exercises. In order to acquaint the participants with the basic ITL and TDD skills, they were shown how to perform micro-slicing, unit testing with JUnit, and the programming-testing-refactoring cycles of ITL and taught the testing-programming-refactoring cycles of TDD. The training sessions included one hour of unit-test training and one hour of TDD training. The training was complemented with: (1) TDD and ITL "Randori" katas (seven and a half hours), where subjects had to apply the concepts learned in the seminar and to develop small applications in groups; and (2) "Solo" sessions (four and a half hours), where subjects had to perform small tasks by individually applying the concepts learned during the session.

Our experiment uses a within-subjects design in which the assignment of tasks to treatments was counterbalanced in order to rule out the impact of subjects and tasks on the assessment of the development approaches. Four different sessions were conducted within the experiment and the subjects applied ITL and TDD in non-consecutive sessions. ITL was applied in the first and third sessions, while TDD was applied in the second and fourth sessions. The time allocated to the implementation of the experimental tasks was 135 minutes each.

Participants were trained in and practised ITL, and then performed the ITL experimental task. Afterwards, the participants were trained in and practised TDD, and then performed the TDD experimental task. In this manner, we assured that there was no leakage from the TDD training to the ITL treatment. For the second two sessions, participants were already acquainted with both development approaches.

Its specification is broken down into 13 fine-grained subtasks. Each subtask of BSK contains a short, general description, a requirement specifying what each subtask is supposed to do, and an example consisting of an input and expected output. The task is further subdivided into 13

We used such test suites to measure the quality of the solutions handed in by the subjects participating in the experiment.

A one-week seminar on TDD was held at the Universidad Polit\'ecnica de Madrid (UPM) in March 2014. A total of 18 graduate students took part in the seminar. They all had a varying range of experience in software development and unit testing skills. All subjects were studying for a master's-level degree in computer science or software engineering at the Universidad Polit\'ecnica de Madrid (UPM). Master's students were free to join the seminar in order to earn extra credits for their degree programme. The seminar was not graded.

Participants were duly informed that they were taking part in an experiment, that their data were totally confidential, and that they were free to drop out of the experiment whenever they liked. Two subjects dropped from the experiment after the first experimental session, which left us with a drop-out rate of 12.5 per cent. Another two subjects did not deliver any working solution along the experimental sessions, and thus we had to remove them from the final dataset. Thus, after pre-processing, a total of 14 subjects made it to the analysis phase. 


\begin{table}[h!]
\caption{Subjects' years of experience with Java.}
\label{subjects_experience_java}
\begin{center}
\begin{tabular}{l|c|c|c|c|c}
    \hline
    \textbf{Variable} & \textbf{N} & \textbf{Mean} & \textbf{Median} & \textbf{Mode} & \textbf{SD}\\ \hline \hline
    Experience Academia  &12& 2.83& 3  & 1 & 1.801 \\\hline
    Experience Industry  &11& 2.45& 2  & 0 & 3.045 \\\hline
\end{tabular}
\end{center}
\end{table}


The participants also filled in information regarding their educational background and previous attendance to TDD courses. Two subjects dropped from the experiment after the first experimental session. This left us with a drop-out rate of 12.5 per cent. Another two subjects did not deliver any working solution along the experimental sessions, and thus we removed their data from the final dataset. After pre-processing, a total of 14 subjects made it to the analysis phase.  

Some of those 14 subject failed to answer the questionnaire. As Table \ref{subjects_background} shows, all the subjects that completed the questionnaire had a background in computer science and worked mainly as developers (8). None of the subjects had any previous experience with TDD. Most of the subjects had previous experience with Eclipse (9) or NetBeans (9), while others had previous experience with other tools (3). The most used unit testing tool was JUnit (7), even though a few subjects never used any testing tools (2) or had experience with other tools such as NUnit (1). 

\begin{table}[h!]
\caption{Subjects' background.}
\label{subjects_background}
\begin{center}
\makebox[\linewidth]{
\begin{tabular}{l|c|l|l|l|l}
    \hline
    \textbf{Variable} & \textbf{N} & \multicolumn{4}{c}{\textbf{Values}}\\ \hline \hline
    Qualifications &13& BSc. CS (6) & MSc. CS (7) & - & - \\\hline
    Professional Experience &14& Developer (8) & Teacher (2) & Analyst (1) & Others (3) \\\hline
    Previous Training in TDD &14 & No (14) & -  & - & - \\\hline
    Currently Used IDE &14& Eclipse (9) & NetBeans (9) & Visual Studio (2) & Others (1) \\\hline
    Unit Testing Tool &9& JUnit (7) & None (2) & NUnit (1) & - \\\hline
\end{tabular}}
\end{center}
\end{table}

Ordinal scales were used to measure previous programming, unit testing, Java, JUnit and TDD experience. 


The data collected in the pre-test questionnaire provided information about the sample participating in our experiment. Our sample belongs to a developer population with medium programming experience (less than 10 years), moderate Java experience (less than five years) and limited experience with unit testing, JUnit, and TDD (less than two years).


\subsection{Subjects}



\subsection{Instrumentation}

The participants performed the experimental tasks on an infrastructure that was embedded within a virtual machine (VM) image using Oracle VM VirtualBox \cite{oracle2015virtualbox}. The image included the Windows 7 operating system, a web browser, Eclipse Helios \cite{eclipse2016} as the development environment, and JUnit 4.3 as the installed unit-testing framework.

This VM was set up in order to ease data collection later on and to guarantee consistency between the packages created by the subjects to deliver their solutions. Furthermore, the use of a VM ensures that all subjects apply the same technologies throughout the experiment and that differences in metrics are not due to different programming environments. 

The main instrument used to extract the QLTY metrics were test cases. A test suite composed of test cases was written by the experimenters for MR, MF and SDK, whereas the BSK test cases were reused from \cite{fucci2013replicated}. 

We provided the subjects with Java project stubs for each of the tasks (MR, BSK, MF and SDK). A hard copy of the task specifications was delivered to the subjects along with the stub. A pre-test questionnaire in Google Surveys was used to collect demographic information about the subjects. It was handed out on the first day in advance of the experimental sessions.

\subsection{Data Collection and Measurement Procedures}

The data collected for each subject included project folders consisting of production and test code and daily snapshots of the VM image. The raw data (code) collected from each participant's computer were stored on hard drives located on site. 

To measure the response variable, a single experimenter executed the test suite associated with each task on the production code of every participant. We stored the number of assert statements passing and failing during this execution as a baseline measure. The same experimenter then computed the QLTY metric. This measurement was double-checked by a second researcher in order to ensure data consistency and that the procedure was followed consistently.



Remember that, in this experiment, we are interested in studying the effect of different factors:
\begin{itemize}
    \item{Development Approach: do the different development approaches (TDD and ITL) have any influence on the outcomes? }
    \item{Development Approach by Task: do either ITL or TDD perform similarly across the different tasks (BSK, MR, MF and SDK)?}
\end{itemize}

We include the following factor in order to reduce the variability of the fitted linear model:
\begin{itemize}
    \item{Task: do the tasks (BSK, MR, MF and SDK) under development have any influence on the outcomes?}
\end{itemize}


\section{Findings}
\label{eight}

This section is organized according to the research questions listed in Section \ref{research_objectives}. Remember that these findings apply to highly committed programmers\footnote{Participants volunteered for the TDD seminar.} with no previous TDD experience developing toy tasks in the Java programming language.

\subsection{Do TDD and ITL perform similarly in terms of quality?}

We cannot reject the null hypothesis for Development Approach with regard to QLTY: \textbf{neither TDD nor ITL works significantly better than the other}. 

\subsection{Do TDD and ITL perform similarly in terms of quality across tasks?}

We cannot reject the null hypothesis for the Development Approach*Task interaction. Thus, \textbf{the differences between ITL and TDD are non-statistically significant across tasks}. This non-significance might be due to the larger sample size required to achieve significant interactions: rather observable variations in effect sizes' magnitude (i.e., medium to large effect size) and sign have been observed across tasks. Indeed, TDD appears outperform ITL for quality in MR and BSK; whilst the opposite seems true in MF and SDK. Furthermore, the magnitude of the differences between ITL and TDD for SDK are larger than those for MR, BSK and MF. Thus, \textbf{the task that is being developed seem to impact both the magnitude and the sign of the differences in QLTY between TDD and ITL}.

In Table \ref{summary_research questions}, we show a summary of the research questions and answers.

\begin{table}[h!]
\small
\caption{Summary of research questions, answers and implications for TDD experiments.}
\label{summary_research questions}
\begin{center}
\begin{tabular}{p{4cm}|p{6cm}} \hline
    \textbf{RE2.RQx} &\textbf{Answer} \\ \hline \hline
    RE2.RQ1. Do TDD and ITL perform similarly in terms of quality? & TDD and ITL appear to behave similarly.  \\ \hline
    RE2.RQ2. Do TDD and ITL perform similarly in terms of quality across tasks? & Task seems to moderate the effect of development approach on quality: ITL outperforms TDD in MF and SDK, whilst the opposite is true for MR and BSK. \\ \hline
\end{tabular}
\end{center}
\end{table}


****************************************************

and our replication (i.e., \textit{RE2} onwards). We provide an overview of BE's and RE1's settings, and a more detailed description of RE2's settings.


\\








BE's quality metric suffers from a main shortcoming, namely, that the weight of each user story makes QLTY subjective. This is because user stories' weights depend upon the test suite implementer. Also because the threshold for considering a user story as delivered (i.e., 50 per cent) is subjective.

Again, the threshold of 50 per cent is not fully argued throughout the article. As in BE, QLTY is still subjective. 


\textbf{RE2}'s test suite and BSK specifications were identical to those in RE1 \cite{fucci2013replicated}. However, 


\textbf{RE2}'s laboratory was also similar. In particular, 


\subsection{Summary of Settings: Differences and Commonalities}
Table \ref{tab:settings_baseline_replications} summarizes the settings of BE, RE1 and our replication (RE2). The changes made in one replication with regards to its predecessor are highlighted in italics.

\begin{table}[h!]
\begin{adjustwidth}{.60in}{-.10in} 
\begin{center}
\caption{Settings of the baseline experiment and replications.}
\label{tab:settings_baseline_replications}
\makebox[\linewidth]{
\begin{tabular}{ l | p{3cm} | p{3cm} | p{3cm} } \hline
\textbf{Aspect} & \textbf{BE} & \textbf{RE1} & \textbf{RE2}  \\ \hline \hline
\textbf{Factors} & Dev. Approach  & Dev. Approach  & Dev. Approach, Task  \\ \hline
\textbf{Treatments} & TDD vs. ITL &  TDD vs. ITL & TDD vs. ITL\\ \hline
\textbf{Response variables} & QLTY &  QLTY & QLTY \\ \hline
\textbf{Metrics} & 50\% threshold \& Weighting  &   \textit{50\% threshold} & \textit{-}\\ \hline \textbf{Design} & Between-subjects design (AB) &  Between-subjects design (AB) & \textit{Within-subjects}
design (ABAB) \\ \hline
\textbf{Subjects} & 13 ITL/11 TDD  &  20 (4 pairs, 16) ITL/ 27 (7 pairs, 20) TDD & 18 \\ \hline
\textbf{Experimental units} & 24  &  47 & 72  \\ \hline
\textbf{Type of subjects} &  Undergraduates &  \textit{Undergraduates} and \textit{Graduates} & \textit{Graduates} \\ \hline
\textbf{Training} & Junior \textit{object-oriented} programming course &  Software \textit{quality and testing} course & \textit{TDD} course\\ \hline
\textbf{Training duration} & Not specified &  6 days/3 hours & 5 days/6 hours\\ \hline
\textbf{Training protocol} & Training in one technique before experimental session (ITL/TDD) & Training in both techniques before experimental session (ITL/TDD) & Training in one technique before experimental session (ITL/TDD) \\ \hline
\textbf{Tasks} & BSK (105 test cases) &  BSK (\textit{48} test cases) & BSK (48 test cases), \textit{MR, MF,} and \textit{SDK}\\ \hline
\textbf{Task Duration} & +8 hours &  3 hours  & 2.25 hours\\ \hline
\textbf{Laboratory} & Inside and outside & \textit{Inside} & Inside \\ \hline
\textbf{Prog. Language} & Java &  Java & Java\\ \hline
\textbf{Environment} & Eclipse, JUnit, CVS &  Eclipse, JUnit & Eclipse, JUnit\\ \hline
\textbf{Stub} & No &  \textit{Yes}  & Yes\\ \hline
\end{tabular}}
\end{center}
\end{adjustwidth}
\end{table}

To ease the measurement of quality, we up-front designed the user stories, test cases and assert statements for each task.

 to improve operationalization. This may increase the construct validity of the replications.
 
 \subsection{Threats to Validity Across Replications}

It also extends BE's and RE1's goal of studying the effectiveness of TDD---by also allowing the investigation of the effect of task on results. This way its possible overcoming mono-operation bias. 

We ran into an extra threat to validity in RE2: carry-over. In particular, subjects might experience carry-over from ITL to TDD. However, this carry-over to TDD is identical for all the subjects, and thus, we cannot determine its impact on results.

Thus, $QLTY_{i}$ still varies between 50 per cent and 100 per cent.

 In other words, we observed similar results whenever subjects were only allowed to develop within the laboratory (ITL$<$TDD), whilst an opposite effect was apparent when subjects were allowed to develop outside the laboratory (ITL$>$TDD).
 
 In general, subjects applying TDD achieved results of more consistent quality (lower variability) for MR, BSK and MF. This finding also holds for RE1 and BE. 

There are two possible explanations for this lower variability:
\begin{enumerate}
    \item{This lower variability in RE1 might be due to the fact that there are more subjects in the TDD group (27 subjects assigned to TDD against 20 to ITL), which may have decreased the variability for quality. However, as the same applies in RE2, where the number of subjects is equal across treatments, this hypothesis must be rejected. Furthermore, there are more subjects assigned to TDD than ITL in BE (13 vs. 11, respectively), which provides further evidence for rejecting this explanation.}
    \item{BSK may have intrinsic properties leading to a lower variability with TDD than with ITL; however, as the same applies in RE2 with MR and MF, we must again reject this hypothesis.}
\end{enumerate}

Here, we hypothesize that cause of the lower observed variability could be the more "rigid" TDD process: subjects are required to plan a test of a small chunk of functionality in advance. On the contrary, the step of defining a test in ITL, used as a control treatment, is more subjective. Therefore, participants might be tempted to continue coding without testing for longer periods. This difference in testing timing or process "rigidity" might explain why subjects do not deviate much from each other: they take similar "baby steps" to implement their solutions. 

Certainly, even though the mean quality of the solutions developed with ITL was slightly larger than the mean quality achieved with TDD, TDD produces smaller deviations and thus has more consistent effects on quality. Such result may be worth considering, as it would make TDD much more appealing to industry from that point of view. Indeed, even though ITL could achieve a small improvement over TDD in mean quality, if the variability is much greater with ITL than with TDD, professionals might prefer the safe option (i.e., choose to use TDD as the range of expected quality is more accurate than with ITL, and quality would eventually be less disperse: there is less of a chance of being in the low quartiles for quality). Given the practical implications of a lower variability, we believe that this finding deserves further research.

Multiple experiments have compared the performance of TDD against other development approaches such as the waterfall or iterative-test-last (ITL) methods. However, the results so far have been largely heterogeneous and inconclusive. The different elements changed along the experimental path and the materialization of various threats to validity may have contributed towards the observed heterogeneity of results.

In this research, we conduct a replication of an already replicated TDD experiment and rely on similar treatments, developer expertise, technological environment and constructs. Furthermore, we mature the evidence from the baseline experiment and the previous replication with the aim of overcoming their main threats to validity and ensuring that the results are independent of the settings.

Specifically, our replication overcame some of the threats to validity present in both the baseline and the replication: (1) the usage of just one task (we used four different tasks); (2) application of only one development approach (all subjects apply both development approaches twice); (3) metrics shortcomings; (4) generalization problem caused by undergraduates (participants in our replication are graduate students about to start a professional career).

Furthermore, we follow the previous replication to overcome some specific threats to the validity of the baseline experiment: (1) randomization to treatments based on ad-hoc skills (every subject applies all treatments in our replication); (2) remote work outside a controlled environment (in both replications, all subjects work from the laboratory) (3) subjective weighting element included within the operationalization of the quality metric (in both replications, such element is removed).

We further set out to avoid some threats to the validity of the previous replication that did not apply to the baseline experiment: (1) confounding of pair programming and subject type (undergraduates and graduates) with development approach and (2) training leakeage between ITL and TDD.

In our replication, TDD appears not to have a statistically significant impact on quality against ITL. This finding is identical across all three replications. However, the magnitude of the results seems inconsistent across experiments: ITL seems to outperform TDD in the baseline experiment, whilst TDD outperforms ITL in the previous replication and our replication.

The directionality of the statistical test did not have an impact on the results. However, programming outside the laboratory, stub provision, the allocation of subjects to treatments, the difficulty element of the quality metric and mono-operation bias may have had an impact on the outcomes. Furthermore, we noticed that TDD experiments might be influenced by the usage of tailored-to-technique tasks or specifications. This could lead to mistaken conclusions or hasty recommendations on the applicability of the techniques in wide-ranging contexts. 

After performing a replication, we managed to mature the evidence found in the baseline and the previous replication and refine various points with regard to the performance of TDD:
\begin{enumerate}
    \item{TDD appears to behave differently to ITL across the different tasks for quality: TDD behaves better than ITL for some tasks and vice versa for others.}
    \item{Task appears to be a statistically significant factor for quality. In other words, the task being developed has a great influence on quality, regardless of the development approach that is being used.}
    \item{The variability observed for quality with TDD generally appears to be lower than with ITL: we suggest that this might be a result of the reversed short intervals of coding and testing that TDD imposes on the subjects and a greater conformance with the technique than with ITL (where subjects might delay testing until they find some functionality has been implemented).}
\end{enumerate}

By means of replication, we have built on previous work and helped to strengthen the reliability of the findings. A new replication has revealed that various moderator variables (i.e., programming outside the laboratory, stub provision, subject allocation to treatment, implementation details of the quality metric and task) might have had an impact on the results of previous experiments, suggesting that researchers shall carefully address the selection of such elements within their experiments. We would like to draw attention to the many variables potentially having an impact on the outcomes of TDD experiments that have yet to be discovered. Likewise, we suggest that these variables are largely responsible for causing the great variability across experimental results on TDD behaviour. Specifically, we encourage TDD experimenters to use multiple tasks since they appear to have a considerable effect on experimental outcomes.

Due to the large heterogeneity of results observed across experiments in Software Engineering, here we encourage researchers to replicate as close as possible their experiments (e.g., sharing experimental tasks, treatment operationalizations, programming environments etc.) with the aim of "coupling" experiments' results and allowing the elicitation of moderators from experiments' settings differences. Detecting, correcting and building on previous threats to validity may give insights to fellow researchers on the impact that certain 'a-priori unnoticed' elements may have on their outcomes. Uncovering moderator variables likely to influence the results across groups of experiments shall be a central aspect of a thorough assessment of the joint results and shall drive the execution of future research.

BE and RE1 test the hypothesis that TDD is superior to ITL in terms of QLTY (and thus, use a one-tailed test). We eliminate this directionality to make an impartial comparison among them (because there is no theory saying that TDD is superior to ITL, and the evidence in the literature is contradictory).


The benefits of replication may be more salient in contexts of heterogeneous results (i.e., when the differences across experiments' results are larger than expected by natural variation \cite{borenstein2011introduction}). This is because heterogeneity might have been introduced not only by the changes made across the experiments (e.g., changes in the experimental tasks), but also because of the materialization of the experiments' threats to validity.

We purposely choose this illustrative example due to the large heterogeneity of results observed in the literature. Particularly, all possible outcomes (positive, negative, and neutral) have been reported for the effectiveness of TDD in terms of quality \cite{rafique2013effects}.
